A Timed Obstruction Logic for Dynamic Game Models

Real-time cybersecurity and privacy applications require reliable verification methods and system design tools to ensure their correctness. Many of these reactive real-time applications embedded in various infrastructures, such as airports, hospitals, and oil pipelines, are potentially vulnerable to malicious cyber-attacks. Recently, a growing literature has recognized Timed Game Theory as a sound theoretical foundation for modeling strategic interactions between attackers and defenders. This paper proposes Timed Obstruction Logic (TOL), an extension of Obstruction Logic (OL), a formalism for verifying specific timed games with real-time objectives unfolding in dynamic models. These timed games involve players whose discrete and continuous actions can impact the underlying timed game model. We show that TOL can be used to describe important timed properties of real-time cybersecurity games. Finally, in addition to introducing our new logic and adapting it to specify properties in the context of cybersecurity, we provide a verification procedure for TOL and show that its complexity is PSPACE-complete, meaning that it is not higher than that of classical timed temporal logics like TCTL. Thus, we increase the expressiveness of properties without incurring any cost in terms of complexity.

==> mainproperties.tex <==
\section{Main Properties}\label{sec:properties}
In this section, we first prove some remarkable semantic equivalences between OL formulae. We then show that the satisfaction relation and the memoryless satisfaction relation  coincides. 


Let $\M=\tuple{S,R,\mathcal{L},\mathsf{C}}$ be a model. We recall that if $s$ is a state $post(s)$ and $pre(s)$ denote, respectively, the set of successors of $s$ and the set of predecessors of $s$. Given a set of states $A$, we define $Pre(A)=\bigcup_{s\in A} pre(s)$. 

If $s$ is a state, $n$ a natural number, and $A$ a set of states, we write $\blacktriangleright(s,n,A)$ whenever $(\sum_{s'\in A} \mathsf{C}(\tuple{s,s'}))\leq n$. If $A$ is a set of states, $\blacktriangledown(n,A)$ denotes the subset of $S$ defined by $\set{s\in Pre(A) \, : \,  \blacktriangleright(s,n,\overline{A})}$.  Let $\varphi$ be any formula:  $\sem{\varphi}^\M$ denotes the set of states of $\M$ verifying, $\varphi$, i.e., $\sem{\varphi}^\M=\set{s\in S \, : \,  \M,s\models \varphi}$. We omit the superscript $\M$ when the model is clear from the context. We are now ready to characterize the set of states satisfying a formula $\naww{\sabotage_n}\next \varphi$. 


\begin{proposition}\label{prop:1}
    For every model $\M$, state $s$, and formula $\varphi$ we have that  $\M,s\models \naww{\sabotage_n}\next \varphi$ if and only if $s\in \blacktriangledown{(n,\sem{\varphi}))}$. 
\end{proposition}
\begin{proof}

For the  $(\Rightarrow)$-direction:  suppose that $s\in \sem{\naww{\sabotage_n}\next \varphi} $, thus there is a n-strategy $\strat$  such that for all $\pi\in Out(s,\strat)$ we have that $\M,\pi_2 \models \varphi$. Suppose, to reach a contradiction, that $s\notin \blacktriangledown(n,\sem{\varphi})$. This could either mean that $s\not\in Pre(\varphi)$ or that $s\in Pre(\varphi)$ and that $\sum_{s'\in \overline{\sem{\varphi}}}\mathsf{C}(s,s') > n$. In the first case, we immediately obtain a contradiction. In the second case, we remark that any n-strategy can deactivate a subset of directed edges whose cost is at most $n$. Thus given any n-strategy $\strat'$ there is a path $\pi \in Out(s,\strat')$ such that $\pi_2\in \overline{\sem{\varphi}}$, which contradicts that $\M,s\models \naww{\sabotage_n}\next\varphi$. 
 	
For the  $(\Leftarrow)$-direction:  suppose that $s \in \blacktriangledown(n,\sem{\varphi})$. By definition, this means that $s\!\in\! Pre(\sem{\varphi})$  and that if $e_1,\ldots,e_n$ are all the edges from $s$ to $\overline{\sem{\varphi}}$, then $(\mathsf{C}(e_1) + \cdots + \mathsf{C} (e_n)) \!\leq\! n$.
Thus, a n-strategy verifying $\naww{\sabotage_n}\next \varphi$ is readily obtained by selecting the set $\set{e_1,\ldots, e_n}$ given the history $h=s$, and the empty-set for any other history $h'$.  
\end{proof}

In the next proposition, we provide the fix-point characterization for the OL operators. 

\begin{proposition}\label{lemma:1}
    For any two formulae $\varphi$ and $\psi$ we have that: 
    \begin{enumerate}
       \item\label{equiv:2} $\naww{\sabotage_n}(\varphi \until \psi)\equiv \psi \vee (\varphi \land \naww{\sabotage_n}\next( \naww{\sabotage_n}(\varphi \until \psi)))$;
       \item\label{equiv:1} $\naww{\sabotage_n} (\varphi \release \psi) \equiv \psi \land  (\varphi \vee  \naww{\sabotage_n} \next (\naww{\sabotage_n} (\varphi \release \psi)))$.
    \end{enumerate}
\end{proposition}
\begin{proof}
 We only prove~(\ref{equiv:2}), the proof of~(\ref{equiv:1}) being entirely similar. 
 
 %\begin{itemize}
 %\item[] 
 $(\Rightarrow)$
 Suppose that $\M,s \models \naww{\sabotage_n} (\varphi \until \psi)$, thus there is a n-strategy $\strat$, such that for every $\tau\in Out(s,\strat)$ there is a $j\in \mathbb{N}$ such that $\M,\tau_j \models \psi $ and $\M,\tau_k \models \varphi$ for every $1\leq k < j$.  If $\M, s \models \psi$ then we can conclude, otherwise since $s=\tau_1$ for any $\tau\in Out(s,\strat)$, we must have that $\M,s\models \varphi$ by hypothesis. Consider the n-strategy $\strat'$ defined by: 
 \begin{equation*}
     \strat'(h)= \begin{cases}
        \strat(h') & \text{if $h'=sh$ and $h'\sqsubset \tau $ for $\tau\in Out(s,\strat)$} \\
        \emptyset & \text{otherwise}.
     \end{cases}
 \end{equation*}
 
  Let $\mathcal{C}=\set{s' \, : \,  \exists \tau \in Out(s,\strat) \text{ s.t. } \tau_2=s'}$; 
	 given any $s'\in \mathcal{C}$  we clearly have that  $\rho \models \varphi \until \psi $ for any $\rho\in Out(s',\strat')$. We deduce that $\M,s'\models \naww{\sabotage_n} \varphi \until \psi$ (the Demon can use the above defined n-strategy $\strat'$) and since the Demon can get to any of the $s'$ by disabling the successors of $s$ disabled by $\strat$ we conclude that $\M, s \models \naww{\sabotage_n} \next ( \naww{\sabotage_n} (\varphi \until \psi))$. 	
	
	
	
 %\item[]
 $(\Leftarrow)$ Suppose that $\M,s \models \psi \vee (\varphi \land \naww{\sabotage} \next (\naww{\sabotage}(\varphi \until \psi )))$. If $\M,s \models \psi$ then we can conclude.  Otherwise $\M,s \models \varphi$ and $\M,s \models \naww{\sabotage_n} \next (\naww{\sabotage_n}(\varphi \until \psi ))$. By the definition of satisfaction, this means that there  is a  n-strategy $\strat$ such that $\M,\rho_2 \models \naww {\sabotage} \varphi \until   \psi $ for any $\rho\in Out(s,\strat)$.  By applying again the definition of satisfaction, we get that there is a n-strategy $\strat_{\rho_2}$ such that for every $\tau\in Out(\rho_2, \strat_{\rho_2}) $ we have that $\M, \tau_k  \models \psi$ for some $k\geq 1$ and $\M,\tau_j \models \varphi$ for any $1\leq j  < k$. 
 We define another n-strategy $\strat''$ by 

 \begin{equation*}
     \strat''(h)= 
     \begin{cases}
         \strat(h) & \text{if $h=s$}\\
         \strat_{\pi_2}(h') & \text{if $h'=s h$ and $h \sqsubset \tau$ for} \\ & \text{$ \tau\in Out(\pi_2,\strat_{\pi_2})$ and $\pi\in Out(s,\strat)$} \\
         \emptyset & \text{otherwise}
     \end{cases}
 \end{equation*}
 
   By the definition of $\strat''$, we obtain that $s\rho\in Out(s,\strat'')$ implies $\rho\in Out(s,\strat_{\pi_2})$ for some $\pi \in Out (s, \strat)$.  Now: suppose that there is a $\tau\in (s,\strat'')$ such that (1)  $\M, \tau_j \not\models \psi$ for all $j\in \mathbb{N}$ or  such that  (2)  $\M, \tau_k \models \psi$ for  some $k\in \mathbb{N}$, and there is a $1 \leq j < k$ such that $\M, \tau_j \not \models \varphi$. In both cases we get a contradiction because such a path also belongs to $Out(\pi_2,\strat_{\pi_2})$ for some $\pi\in Out(s,\strat)$. We can thus finally conclude that $\M,s\models \naww{\sabotage_n} (\varphi \until \psi)$ as we wanted. 
 %\end{itemize}
\end{proof}



Let $\M=\tuple{S,R, \mathcal{L},\mathcal{C}}$ be a model and $\varphi$, $\psi$ be two formulae. Consider the two monotone functions $\mathsf{R^n}_{\varphi,\psi}$ and $\mathsf{U^n}_{\varphi,\psi}$ from $2^S$ to itself, for any subset $X$ of $S$, defined by: 
\begin{equation}
    \mathsf{U}^n_{\varphi,\psi}(X)  = \sem{\psi}^\M \cup (\sem{\varphi}^\M \cap \blacktriangledown (n, X)) 
\end{equation}
\vspace{-2em}
\begin{equation}\label{eq:release}
    \mathsf{R}^n_{\varphi,\psi}(X)  = \sem{\psi}^\M \cap (\sem{\varphi}^\M \cup \blacktriangledown (n, X)) 
\end{equation}
\noindent we can prove the following. 

\begin{thm}\label{thm:fixpoint}
    For every model $\M$ and two formulae $\varphi$ and $\psi$: 
    \begin{enumerate}
        \item\label{fixpoint:2} $\sem{\naww{\sabotage_n} (\varphi \until \psi)}^\M$ is the least fix-point of  $\mathsf{U}^n_{\varphi,\psi}$;
        \item\label{fixpoint:1} $\sem{\naww{\sabotage_n} (\varphi \release \psi)}^\M$ is the greatest fix-point of $\mathsf{R}^n_{\varphi,\psi}$. 
    \end{enumerate}
\end{thm}
\begin{proof}
We only give a proof of~(\ref{fixpoint:1}). In virtue of Propositions~\ref{prop:1} and~\ref{lemma:1} it is clear that $X=\sem{\naww{\sabotage_n}(\varphi \release \psi)}^\M$ is a fix-point of $\mathsf{R}^n_{\varphi,\psi}$. Let $Y$ be any other fix-point of the function. If $Y=\emptyset$ the result trivially holds. Otherwise, we show that  given $v\in Y$ we have that  $v\in X$. Since $Y$ is a fix-point of the function, we have that $v\in \sem{\psi}$ and either  $v\in \sem{\varphi}$ or $v\in \blacktriangledown(n, Y)$. If this last case,  for the set  $E_v$ of edges whose source is $v$ and whose target is not in $Y$ we have that $(\sum_{e\in E_v} \mathcal{C}(e))\leq n$. We define an n-memoryless  strategy $\strat$ by 

\begin{equation*}
    \strat(v) = 
    \begin{cases}
         E_v & \text{ if } v\in \sem{\psi} \cap \blacktriangledown (n,Y) \\
         \emptyset & \text{ otherwise}
    \end{cases}
\end{equation*}

Now consider a path $\rho\in  Out(v,\strat)$ for $v\in Y$.   %By construction of $\strat$, we have that for any $i\in \mathbb{N}$, $\rho_i \in Y$ implies that either $\rho_i \in {\varphi}^\M $ or $\rho_{i+1} \in \sem{\psi}$.
Since $\rho_1=v\in Y$, let $\mathcal{X}=\set{k\geq 2 \, : \, \rho_k\not\in Y}$. If $\mathcal{X}$ is empty, then each $\rho_i\in \sem{\psi}$, otherwise let $j\geq 2$ be the smallest integer such that $\rho_j\not\in Y$. Suppose to reach a contradiction that $\rho_{j-1} \notin \sem{\varphi}$. Since $\rho_{j-1}\in Y$ and $\rho_j\notin \sem{\varphi}$ we must have that $\rho_j\in \sem{\psi} \cap \blacktriangledown (n,Y)$.   Thus, given any $\pi\in Out(\rho_j, \strat)$ we obtain that $\pi_2\in Y$. Since $\strat$ is memoryless, we obtain a contradiction  because $\pi_2=\rho_j$ for some $\pi \in Out(\rho_{j-1},\strat)$.  
\end{proof}



As we have anticipated, we now show that the set of formulae that are true under the satisfaction relation and the memoryless satisfaction relation coincides. 


\begin{lemma}
    For any formula $\varphi$, for any model $\M$ and state $s$: if $\M,s\models\varphi$ then $\M,s\models_{r}\varphi$.
\end{lemma}
\begin{proof}
    The proof is by induction on the structure of $\varphi$. Remark that for the case $\varphi=\naww{\sabotage_n} \psi_1\release \psi_2$, we showed in Theorem~\ref{thm:fixpoint} how given any $v$ belonging to a fix-point of the function~$\mathsf{R}^n_{\psi_1,\psi_2}$, it is possible to construct a n-memoryless strategy $\strat$ such that all paths in $Out(v,\strat)$ satisfies $\psi_1 \release \psi_2$. As a consequence, we only detail the cases $\varphi=\naww{\sabotage_n}\next \psi$ and $\varphi= \naww{\sabotage_n} (\psi_1 \until \psi_2)$. The proof for the $\naww{\sabotage_n} (\psi_1 \until \psi_2)$ case is inspired by the one presented in~\cite{KnapikPetrucciJamrogaTimed}. 
    %\begin{itemize}
        %\item 
        
    If $\varphi=\naww{\sabotage_n}\next \psi$, $\M,s\models \varphi$ iff there is a  n-strategy $\strat$ such that $\tuple{\M,\rho_2}\models \psi$ for all $\rho\in Out(s,\strat) $. By induction hypothesis, $\M,\rho_2 \models \psi$.  Consider the n-strategy $\strat'$ such that $\strat'(h)=\strat(s)$ if $last(h)=s$ and $\strat'(h)=\emptyset$ otherwise. This latter n-strategy is memoryless, and for any $\tau\in Out(s,\strat')$, $\tau_2=\rho_2$ which establish the wanted result. 
    \iffalse 
    if $\varphi=\naww{\sabotage_n}\globaly \psi$ then $\M,s\models \varphi$ iff there is a n-stratety $\strat$ s.t.  for any $i\in \mathbb{N}$, $\M, \rho_i \models \psi $ for every $\rho\in Out(s,\strat)$. Given an history $h=s_1,\ldots,s_n$ of $S$, we say that $h\in H^\strat_{s'}$ iff  $s_n=s'$, all the $s_i$ are distinct and $h\sqsubset \rho$ for some $\rho \in Out(s,\strat)$.  Given $H^\strat_{s'}$, we  choose one of its element that is minimal with respect to the prefix order, and denote it $h^{min}_{s'}$. We now define a memoryless n-strategy $\strat'$ by 
       \begin{equation*}
            \strat'(s') \begin{cases}
                \strat(h^{min}_{s'}) & \text{if $H^\strat_s\neq \emptyset$}
                \\
                \emptyset & \text{otherwise}
            \end{cases}
        \end{equation*}
        
        
         Let $h'$ be any finite sequence of states that is the prefix of some path in $Out(s,\strat')$;  we show that for any $i\leq |h|$,  $h_i=\rho_j$ for some $j\in \mathbb{N}$ and $\rho \in Out(s,\strat)$ by induction on $|h|$.
        If $|h'|=1$ then $h=s$ and  the result is clear. Suppose that the results holds for each $h''$ such that $|h''|\leq n$ and let $h'= s_1,\ldots,s_n, s_{n+1}$. If $s_{n+1}=s_i$ for some $i\leq n$, then we are done. Otherwise, $s_{n+1}$ is different from all the $s_i$. By definition, there is a path of the form  $\strat(h^{\min}_{s_n}), s_{n+1}$ over $S$, which implies that $s_{n+1}=\tau_j$ for some $\tau\in Out(s,\strat)$. 
\fi 
%\item

If $\varphi=\naww{\sabotage}\psi_1 \until \psi_2$. Let $\strat$ be a n-strategy such that $\psi_1 \until \psi_2$ holds for any path $\pi\in Out(s,\strat)$. Let $\mathcal{X}=\set{\pi_{\leq k} \, : \,  \pi \in Out(s,\strat) \land \M,\pi_k\models \psi_2 \land \M,\pi_j\models \psi_1 \text{ for all $1\leq j<k$} }$ and $\mathcal{Y}$ its prefix-closure.
Given  $v\in S$, let $h_v$  be a  sequence in  $\mathcal{Y}$ such that $last(h_v)=v$ and $\not\exists h^\star\in \mathcal{Y}$ such that $h_v\sqsubset h^\star$ and $last(h^\star)=v$. Define a n-strategy $\strat_{h_v}$ by: 
\begin{equation*}
    \strat_{h_v}(h)=\begin{cases} \strat(h_v\cdot h'') & \text{ if $h=h'\cdot h''$ and $last(h')=v$ }
    \\
    \strat(h) & \text{otherwise}
    \end{cases}
\end{equation*}
Such a n-strategy associates the same set of edges to any history ending in $v$ and we clearly have that  any path in its outcome set verifies $\psi_1 \until \psi_2$. Repeat the above procedure for any $s'\in S$. After at most $|S|$ steps, we obtain a memoryless n-strategy $\strat'$ in which any path verifies $\psi_1 \until \psi_2$. 
%\end{itemize}
\end{proof}
 By the above lemma and by the fact that any memoryless n-strategy is a n-strategy, one immediately obtains the following. 
\begin{thm}\label{thm:memoryless}
    For any formula $\varphi$, for every model $\M$ and state $s$, we have that  $\M,s\models_{r}$ if and only if $\M,s \models \varphi$.
\end{thm}

